Differentially Private Numerical Vector Analyses in the Local and Shuffle Model

Numerical vector aggregation plays a crucial role in privacy-sensitive applications, such as distributed gradient estimation in federated learning and statistical analysis of key-value data. In the context of local differential privacy, this study provides a tight minimax error bound of $O(\frac{ds}{n\epsilon^2})$, where $d$ represents the dimension of the numerical vector and $s$ denotes the number of non-zero entries. By converting the conditional/unconditional numerical mean estimation problem into a frequency estimation problem, we develop an optimal and efficient mechanism called Collision. In contrast, existing methods exhibit sub-optimal error rates of $O(\frac{d^2}{n\epsilon^2})$ or $O(\frac{ds^2}{n\epsilon^2})$. Specifically, for unconditional mean estimation, we leverage the negative correlation between two frequencies in each dimension and propose the CoCo mechanism, which further reduces estimation errors for mean values compared to Collision. Moreover, to surpass the error barrier in local privacy, we examine privacy amplification in the shuffle model for the proposed mechanisms and derive precisely tight amplification bounds. Our experiments validate and compare our mechanisms with existing approaches, demonstrating significant error reductions for frequency estimation and mean estimation on numerical vectors.

==> comparison.tex <==
\section{Sub-optimality of Existing Mechanisms}\label{sec:comparison}
Existing works on $\epsilon$-LDP numerical vector aggregation can be categorized into two types, that is they do dimension sampling in a data-agnostic manner (e.g., in \cite{Ye2019PrivKVKD,sun2019conditional}) or a data-dependent manner (e.g., in \cite{gu2019pckv}). After that, both types of works follow the same idea of transforming the problem of $\epsilon$-LDP on numerical vector into a problem of $\epsilon$-LDP on categorical data. In this section, we theoretically analyze mechanisms proposed by these works and show their statistical efficiency gap from the optimal rate. 

\subsection{The PrivKV Mechanism}
The seminal work \cite{Ye2019PrivKVKD} on $\epsilon$-LDP key-value data aggregation propose to firstly randomly sample a dimension (from the domain of keys) $j\in[d]$, then applies an $\epsilon$-LDP categorical mechanism on the corresponding (key,value) pair that takes a value from $\{(j,0),(j,1),(j,-1)\}$, where $(j,0)$ means that the key is empty in the key-value data. Recall that $j_-$ and $j_+$ denote events that the $j$-th element of $\mathbf{x}$ (i.e. $\mathbf{x}_j$) equals to $-1$ and $1$ respectively, and a numerical vector $\mathbf{x}$ could be represented in the set form as:
%\vspace*{0.2em}
\small
$$\mathbf{Y}_\mathbf{x}=\{j_-\ |\ j\in[d]\ \text{and}\ \mathbf{x}_j=-1\} \bigcup \{j_+\ |\ j\in[d]\ \text{and}\ \mathbf{x}_j=1 \}.$$
\normalsize
%\vspace*{0.0em}

Essentially, the PrivKV mechanism is equivalent to dividing the population of $n$ into $d$ groups, and each group is employed to estimate $[j_+\in \mathbf{Y}_{\mathbf{x}}]$ and $[j_-\in \mathbf{Y}_{\mathbf{x}}]$ for each $j\in[d]$ with privacy budget $\epsilon$. Since the minimax lower error bound for estimating frequencies on population of $n'$ with privacy budget $\epsilon$ and domain size $d'$ is $\Theta(\frac{d'}{n'\epsilon^2})$ \cite{duchi2018minimax}, the estimation error of $[j_+\in \mathbf{Y}_{\mathbf{x}}]$ and $[j_-\in \mathbf{Y}_{\mathbf{x}}]$ is hence $\Theta(\frac{d}{n\epsilon^2})$, as $n'=\frac{n}{d}$ and $d'=3$. Therefore, its total estimation error of frequencies or mean values of $d$-dimensional vector is: $$\Theta(\frac{d^2}{n\epsilon^2}),$$ 
which has a gap of $\frac{d}{s}$ from the optimal error rate in Theorem \ref{the:setminimax}. Similar methodology and result also hold for the following-up work in \cite{sun2019conditional}.

\subsection{The PCKV Mechanism}
As opposed to sampling a key from the whole domain of $[d]$, the work of \cite{gu2019pckv} proposes to sample a key from existing $s$ keys in a key-value data. Afterwards, an $\epsilon$-LDP categorical mechanism is applied to the corresponding $1$-sparse set-value data, which is equivalent to categorical data with domain size of around $2d$. 

Recall that the minimax lower error bound for estimating frequencies on population of $n'$ with privacy budget $\epsilon$ and domain size $d'$ is $\Theta(\frac{d'}{n'\epsilon^2})$, the total estimation error of scaled $[j_+\in \mathbf{Y}_{\mathbf{x}}]$ and $[j_-\in \mathbf{Y}_{\mathbf{x}}]$ in the PCKV mechanism is hence $\Theta(\frac{d}{n\epsilon^2})$, as $n'=n$ and $d'=2d$. Due to the previous sampling procedure, the scale factor is $s$ and the total variation error is amplified by $s^2$, thus the total estimation error of $[j_+\in \mathbf{Y}_{\mathbf{x}}]$ and $[j_-\in \mathbf{Y}_{\mathbf{x}}]$ in the PCKV mechanism is:
$$\Theta(\frac{ds^2}{n\epsilon^2}).$$
Such an error bound has a gap of $s$ from the optimal error rate in Theorem \ref{the:setminimax}.
